Femto-Caching with Soft Cache Hits: Improving Performance through Recommendation and Delivery of Related Content

Pushing popular content to cheap "helper" nodes (e.g., small cells) during off-peak hours has recently been proposed to cope with the increase in mobile data traffic. User requests can be served locally from these helper nodes, if the requested content is available in at least one of the nearby helpers. Nevertheless, the collective storage of a few nearby helper nodes does not usually suffice to achieve a high enough hit rate in practice. We propose to depart from the assumption of hard cache hits, common in existing works, and consider "soft" cache hits, where if the original content is not available, some related contents that are locally cached can be recommended instead. Given that Internet content consumption is entertainment-oriented, we argue that there exist scenarios where a user might accept an alternative content (e.g., better download rate for alternative content, low rate plans, etc.), thus avoiding to access expensive/congested links. We formulate the problem of optimal edge caching with soft cache hits in a relatively generic setup, propose efficient algorithms, and analyze the expected gains. We then show using synthetic and real datasets of related video contents that promising caching gains could be achieved in practice.

==> discussion.tex <==
In this section, we discuss some shortcomings and possible extensions of our framework.

%\item Generic $u_{kn}$ values. We discussed with Pavlos and it is probably possible to directly treat this as the only case (no need for the ``type 1'' $U$). If not though, we must definitely try to say something about the generic case.

\emph{Incentives for soft cache hits}: In the case of replacement, i.e. when a user asks for A and she gets B, one would argue that the user needs some incentive to accept this. This could potentially be handled in the following ways: (i) if a user has a low cost plan, we can force the user to take B when the network is congested; this might still be preferable as many low cost plans offer very limited or no data at all. (ii) the operator could propose to give B for ``free'' (e.g. not counting in the plan) and let the user decide, or letting the user know that accessing $A$ from the core infrastructure would be slow and choppy, while B might have much better performance. It would be very interesting to model and study if/when this tradeoff would be financially beneficial to the operator. A second interesting case is when a user ``browses'' content in sequence (e.g YouTube). In that case, a replacement ``penalty'' could be avoided. The recommended contents can just be biased to the ones in a cache, and the user is usually willing to follow any of these, as long as they are relevant.% If of course none of the recommended next contents are relevant at all, the user might decide to pick something else or search further.

\emph{User-based recommendations}: \st{Throughout this paper, we have been assuming that the related contents for a requested content item $i$, and their related utilities depend only on item $i$, and not on the user that requested it. In a sense, this relates to \emph{item-item} collaborative filtering, where a new/alternative item is recommended based on its similarity with the requested one. Item-item recommendations have been claimed to offer some advantages compared to \emph{user-user} collaborative filtering%~\cite{Collab-Filter-Sigmetrics2016}
. Nevertheless, one user might be less happy than another, with the same alternative content. On the modeling side, one could take this into account by making $u_{ij}$ a random variable and using its expected value $E[u_{ij}]$ in the objective functions of the respective optimization problems. %One could also try to establish bounds on this approach (e.g., based on the \add{concavity} properties of the objective, using Jensen's inequality). 
Finally, on the recommendation side, a recommendation system could actually combine both types of collaborative filtering to make better recommendations. This would lead to different $\mathbf{U}$ graphs per user (or user clusters), whose integration and impact on our framework is part of future work.} \rem{We address this with the per-user utility/popularity}

%\item (MAYBE) If in the generic problem greedy doesn't perform that close to optimal (how do we know...?) perhaps we can try a heuristic based on our understanding of graphs. \emph{Step 1}: Pick a size K, cluster U into K communities (could do K-means, but I think spectral clustering would work better). This is polynomial time. \emph{Step 2}: In each community, pick the content which covers the most popularity (his + his neighbors). Given that the community sizes will be much smaller than the original problem, this can even be done with brute force. \emph{Step 3}: Now use a *new* catalog of these K contents (the "clusterheads"). Say that these cover 80\% of the total popularity. Ok, for the rest of 20\% you always get it from infrastructure. For the rest of the 80\% you solve the femtocaching problem, but now with this new (hopefully) much smaller catalog. so you should hopefully do better. 
%\item (MAYBE) look at related literature for results related to vertex cover in different types of random graphs. translate them/adapt them for our problem.

\emph{Probabilistic User-SC relationship}: One interesting departure from the standard femto-caching model is if we did not know with probability 1 which BSs a user will see the next day. This essentially gives a probabilistic bipartite graph, where an edge has a weight in $[0,1]$, based on which the content allocation must be performed, optimizing \emph{expected} performance. Such a system could also more realistically capture mobility and related uncertainties of users. \rem{Not only more realistic, but also allows to consider caching in a larger time-scale (i.e., where users move).} It would be interesting to model such a system, in the context of femto-caching with soft cache hits, and study whether the observed performance gains would not vanish under uncertainty.

%\add{ (MAYBE) we could discuss how soft cache hits apply to opportunistic (delayed) access (e.g. summarize the CHANTS result) and maybe PHY-aware caching (the framework of Mobihoc 2015 by Psounis).}



==> related.tex <==
Densification of cellular networks, overlaying the standard macro-cell network with a large number of small cells (e.g., pico- or femto-cells), has been extensively studied and is considered a promising solution for the increasing data demand~\cite{hetnets-commag-2012,femtocells-survey-jsac-2012,hetnets-paradigm-shift}. As this densification puts a tremendous pressure on the backhaul network, researchers have suggested storing popular content at the ``edge'', e.g., at small cells~\cite{femto}, user devices~\cite{femtoD2D,Hui-offloading,sermpezis2014}, or vehicles acting as mobile relays~\cite{vigneri2016}. 

In our work, we complement such approaches, by proposing not only mobile edge caching but also recommendation of the cached contents in order to reduce the demand for non-cached contents. This solution, which we first proposed in the context of mobile (ad-hoc) networks with delayed content delivery~\cite{sch-chants-2016}, as shown both in~\cite{sch-chants-2016} and in the present work, can offer significant gains and alleviate the backhaul networks.

Joint study of caching and recommendation strategies has not been considered before for cellular networks. Some previous works explore the common effect for peer-to-peer networks~\cite{content-recommendation-swarming} and CDNs~\cite{what-should-you-cache-nossdav,cache-centric-video-recommendation}. Specifically, ~\cite{content-recommendation-swarming} studies the interplay between a recommendation system and the performance of content distribution on a peer-to-peer network like BitTorrent. The authors model and analyse the performance, and propose heuristics (e.g., the number of cached copies, or ``seeders'' in BitTorrent) for tuning the recommendation system in order to improve performance and reduce content distribution costs. Although in our work we follow a reverse approach (given a recommendation system and user utilities, we ``tune'' the content caching), it would be interesting to investigate this in the context of cellular networks as well.

~\cite{what-should-you-cache-nossdav} shows that users tend to follow YouTube's suggestions, and despite the large catalog of YouTube, the top-10 recommendations are usually common for different users in the same geographical region. Hence, CDNs can use the knowledge from the recommendation system to improve their content delivery (e.g., by storing in central caches the most appropriate contents). In~\cite{cache-centric-video-recommendation} the authors suggest a recommended list reordering approach that can achieve higher cache hit ratios (for YouTube servers/caches). In particular, they show that performance can be improved when the positions of contents in the related list of YouTube are not changed compared to the previous recommended list.



%%%%%% some copy-paste text from Infocom that contains references%%%%%


%
%This suggests that even though studies assuming a large (CDN-type) cache deep inside the core network give promising hit ratios~\cite{Erman2011}
%
%More than 1TB storage would be needed to just store $0.1\%$ of either one~\cite{tutorial-sigmetrics}. Considering other VoD platforms, YouTube, etc., this number explodes. Even, with a skewed popularity distribution, \emph{local} cache hit ratios would be rather low~\cite{Paschos-misconceptions}. 
%
%
%
%While our problem formulation and analysis takes place in the context of \emph{femto-caching}, the idea of soft cache hits is also applicable to some of the other caching frameworks mentioned earlier. These include caching for opportunistic or delay-tolerant networking~\cite{Hui-offloading,Whitbeck-offloading,vigneri2016}, PHY-aware caching~\cite{Psounis2015, Lau:PhyCache}, or even wired caching, where soft cache hits could offer additional gain factors. 
